Online Semi-Supervised Learning in Contextual Bandits with Episodic Reward

We considered a novel practical problem of online learning with episodically revealed rewards, motivated by several real-world applications, where the contexts are nonstationary over different episodes and the reward feedbacks are not always available to the decision making agents. For this online semi-supervised learning setting, we introduced Background Episodic Reward LinUCB (BerlinUCB), a solution that easily incorporates clustering as a self-supervision module to provide useful side information when rewards are not observed. Our experiments on a variety of datasets, both in stationary and nonstationary environments of six different scenarios, demonstrated clear advantages of the proposed approach over the standard contextual bandit. Lastly, we introduced a relevant real-life example where this problem setting is especially useful.

==> main.tex <==
% % This is samplepaper.tex, a sample chapter demonstrating the
% % LLNCS macro package for Springer Computer Science proceedings;
% % Version 2.20 of 2017/10/04
% %
% \documentclass[runningheads]{llncs}
% %
% \usepackage{graphicx}
% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{hyperref}       % hyperlinks
% \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography

% \newcommand{\theHalgorithm}{\arabic{algorithm}}

% \usepackage{url}
% \usepackage{algorithm}
% \usepackage{algorithmic}
% \usepackage{graphicx}
% \usepackage{amsthm}
% \usepackage{amssymb}
% \usepackage{multicol}
% \usepackage{amsmath}
% \usepackage{wrapfig}

% \newcommand{\argmax}[1]{\underset{#1}{\operatorname{arg}\,\operatorname{max}}\;}
% % Used for displaying a sample figure. If possible, figure files should
% % be included in EPS format.
% %
% % If you use the hyperref package, please uncomment the following line
% % to display URLs in blue roman font according to Springer's eBook style:
% % \renewcommand\UrlFont{\color{blue}\rmfamily}

% \begin{document}
% %
% \title{Online Semi-Supervised Learning in \\Contextual Bandits with Episodic Reward}
% %
% \titlerunning{Contextual Bandits with Episodic Reward}
% % If the paper title is too long for the running head, you can set
% % an abbreviated paper title here
% %

% \author{Baihan Lin\inst{1,2}}
% % \orcidID{0000-0002-7979-5509}}
% %
% \authorrunning{B. Lin}
% % First names are abbreviated in the running head.
% % If there are more than two authors, 'et al.' is used.
% %
% \institute{Center for Theoretical Neuroscience, Columbia University, New York, USA \and
% Zuckerman Mind Brain Behavior Institute, Columbia University, New York, USA \\
% % \and Department of Systems Biology, Columbia University Medical Center, New York \\
% \email{Baihan.Lin@Columbia.edu}\\}

% % \author{Anonymous\inst{1,2}}
% % % \orcidID{0000-0002-7979-5509}}
% % %
% % \authorrunning{Anonymous}
% % % First names are abbreviated in the running head.
% % % If there are more than two authors, 'et al.' is used.
% % %
% % \institute{Anonymous University \and
% % Anonymous Research Institute \\
% % % \and Department of Systems Biology, Columbia University Medical Center, New York \\
% % \email{Anonymous@Anonymous.edu}\\}

% %
% \maketitle              % typeset the header of the contribution
% %
% \begin{abstract}

% We considered a novel practical problem of online learning with episodically revealed rewards, motivated by several real-world applications, where the contexts are nonstationary over different episodes and the reward feedbacks are not always available to the decision making agents. For this online semi-supervised learning setting, we introduced Background Episodic Reward LinUCB (BerlinUCB), a solution that easily incorporates clustering as a self-supervision module to provide useful side information when rewards are not observed. Our experiments on a variety of datasets, both in stationary and nonstationary environments of six different scenarios, demonstrated clear advantages of the proposed approach over the standard contextual bandit. Lastly, we introduced a relevant real-life example where this problem setting is especially useful. (Codes can be accessed at \href{https://github.com/doerlbh/BerlinUCB}{\underline{https://github.com/doerlbh/BerlinUCB}}).

% % \footnote{The data and codes can be accessed at \href{https://github.com/doerlbh/BerlinUCB}{\underline{https://github.com/doerlbh/BerlinUCB}}}


% \keywords{Multi-Armed Bandit \and Contextual Bandit \and Online Learning \and Semi-Supervised Learning \and Online Clustering \and Nonstationary Setting}
% \end{abstract}
% %
% %
% %

% \input{./sec_intro.tex}
% \input{./sec_related.tex}
% \input{./sec_problem.tex}
% \input{./sec_method.tex}
% \input{./sec_results.tex}
% \input{./sec_conclusion.tex}



% \bibliographystyle{splncs04}
% \bibliography{main}

% \end{document}


==> sec_results.tex <==
% \clearpage
\section{Empirical Evaluation}

We evaluated our approach on six synthetic nonstationary online learning scenarios in two datasets: MNIST \cite{lecun1998mnist} and Warfarin \cite{international2009estimation}, and provided a real-life application where the episodic feedbacks are naturally installed: a speaker diarization task with sporadic human interactions as bandit feedbacks. For the synthetic online learning task, in order to simulate an online data stream, we draw samples from each dataset sequentially, starting from the beginning each time we draw the last sample. At each round, the algorithm receives  reward 1 if the instance is classified correctly, and 0 otherwise. We compute both the final cumulative reward and the total number of classification errors as the performance metrics. However,  Warfarin dataset is different, as it was actually produced in a real bandit setting, rather than classification setting.

\textit{Important distinction on Bandit vs. classification feedback}: It is important to keep in mind that the bandit feedback (correct/incorrect classification) makes the classification problem significantly more challenging,  as compared to the standard supervised learning, since the true label is never revealed in bandit setting unless the classification is correct. Thus, the classification accuracy in a bandit setting is expected to be lower than in the supervised learning setting, which is not due to inferiority of bandit decision making algorithm versus classifiers, but due to increased problem difficulty, i.s. the lack of feedback about what the correct decision should have been. Recall that such bandit feedback is often a much more realistic model of agent's interaction with the world, especially in online decision making applications such as online advertisement, clinical trials, and so on, which do not fit into the classical classification framework.

However, for empirical evaluation purposes, it is common to use available classification datasets to simulate an online environment with the bandit feedback  (i.e., simulating the situation where the bandit receives, for example, 1 or 0 for correct or incorrect decision, but is not told what the correct decision should have been when it receives 0; such feedback is different from standard online classification feedback in case of non-binary classification). We use the classification dataset here to create online learning simulation environments.

We now describe some details of the experiments. For MNIST, we took the 5,000 samples from the training dataset to simulate the online bandit with 10 arms corresponding to different digits. For Warfarin dataset, we selected the first 5,000 training samples to simulate the online bandit with 3 arms (classes). As an even more challenging task, we also created a multi-task scenario where a mixture of the MNIST and the Warfarin task are fed in batches.  We extended the set of possible labels (arms) to include 10 labels from MNIST and 3 labels from Warfarin, into a total of 13 arms. We used linear stretching to make the input dimensions equal across the two domains. In another word, for each input, we concatenate the Warfarin features (of size 93) on the back of the MNIST features (of size 784) into a sparse vector of size 877. The algorithm had to assign a label to each input without any information about which domain the input came from.
%Since each dataset had a different number of online iterations (samples), we decided to report the full results as well as the first 8000 iterations (using random subsets of 8000 samples for each domain) to make the results more comparable.


\subsection{Nonstationary Environments}

We simulated six types of nonstationarity using the above datasets (with a batch size of 100). As mentioned before, we assume that the input data arrive in batches, and the data distribution (i.e., the joint distribution of the context and reward) may change across those batches, while remaining stationary within each batch. 
% We used the batch size of 100 and presented average results over multiple runs.  

\vspace{-1em}

\subsubsection{Nonstationary oracle: fixed vs. extendable arms.} Traditional online learning have a fixed number of arms (denoted ``F''). We here considered such a nonstationarity where we start with a single arm, and when new labels arrive new arms are generated accordingly, a problem loosely modelled by the bandits with infinitely many arms \cite{berry1997bandit}. For this setting, we applied an arm expansion process  (denoted ``E''): starting from a single arm (for adding a ``new'' arm), if a feedback confirms a new addition, a new arm is appended to the arm list.
%  outlined in Figure \ref{fig:bandit}

\vspace{-1em}

\subsubsection{Nonstationary oracle: varying episodic rewards.}
Last but not least, we may assume the probability of the reward revealing ($p_r$ in Algorithm \ref{alg:episode}) can change from batch to batch. In another word, the reward feedback can be more frequently revealed in some episode or mini-batch than the others.  

\vspace{-1em}


\subsubsection{Nonstationary context: varying cluster distribution.} 
To simulate changes in the context (input) distribution, we first   clustered all samples in the corresponding  pre-training data subset   into $k$ clusters. Next, we generate a sequence of batches, where each  batch   contained a certain fraction of samples from different clusters, and these fractions were changing across the batches, i.e. the probability distribution of cluster membership was changing, simulating nonstationary input.

\vspace{-1em}

\subsubsection{Nonstationary context: negative images.}
Another type of input  nonstationarity involved introducing negative images as inputs with same semantics but different textures. Namely, with probability $p$, the negative image of the original image was  presented as an input. 
Experiments were performed with this data corruption given by $0 < p < 1$ episodically and randomly assigned for each batch.

\vspace{-1em}

\subsubsection{Nonstationary reward: shuffled class labels.}
 We further explored the multi-task setting by introducing a different type of nonstationary reward, where the class labels were shuffled, i.e. randomly permuted, in each batch.

\vspace{-1em}

\subsubsection{Nonstationary reward: multi-task environment.} Here we assume that input samples come from different domains (tasks), and thus can be associated with different subsets of labels (arms). For example, we combined 5,000 randomly selected training samples from each of the two selected domains, MNIST and Warfarin datasets, and extended the set of possible labels (arms) to include 10 labels from MNIST and 3 labels from Warfarin into a mixed dataset of 10,000 samples of 13 arms. We used linear stretching to make the  input dimensions equal across the two domains. The algorithm had to assign a label to each input without any information about which domain the input came from.


% \begin{figure}[tb]
% \centering
% \vspace{-0.4cm}
%   \includegraphics[width=0.5\linewidth]{Figures/bandits.png}
% \par\caption{Arm expansion process of bandits.}\label{fig:bandit}
% \vspace{-0.1cm}
% \end{figure}
 
%\subsection{Short-term nonstationary environments}

% % Table \ref{table:nonstatAccUnshuffled8000} summarizes our results for the nonstationary online learning setting in the short term (till t = 8,000); it represents the average classification accuracy, where the averaging is done over the total number of iteration and selecting the maximum accuracy from the experiments with three embedding sizes (2,4 and 8). 

% The \textit{universal embedding} achieved the best performance among all methods on all datasets except for Caltech-101 and mixed MNIST/Warfarin datasets, confirming the importance of embedding adaptation in a nonstationary setting. We also observe that, across all datasets, the unsupervised embedding selection (\textit{mini-batch embedding}) performs quite well when the nonstationarity increases in the mixed dataset, underscoring  importance of efficient embedding selection across the data batches in nonstationary environment.

% Overall, based on their mean accuracy in the short term, the top three algorithms were: \textit{universal embedding} (mean accuracy 23.86$\%$), \textit{mini-batch embedding} (mean accuracy 22.58$\%$), \textit{online embedding} (mean accuracy 20.31$\%$), respectively, suggesting that using an adaptive encoding may  be a better strategy than ignoring any unlabeled context history in a standard MAB to directly learn to classify given the original context, i.e. the baseline, which resulted into the worst mean accuracy of 15.99$\%$.


\subsection{Results}

\begin{figure}[tb]
\centering
% \vspace{-0.2cm}
    \includegraphics[width=0.24\linewidth]{Figures/result1_1_none_0p01_1_rew.png}
    \hfill
    \includegraphics[width=0.24\linewidth]{Figures/result1_1_cluster_0p01_1_rew.png} \hfill
    \includegraphics[width=0.24\linewidth]{Figures/result1_1_negative_0p1_1_rew.png} \hfill
    % \includegraphics[width=0.24\linewidth]{Figures/result1_1_reward_0_1_rew.png} \hfill
    \includegraphics[width=0.24\linewidth]{Figures/result1_1_reward_0p01_1_rew.png}
    \includegraphics[width=0.24\linewidth]{Figures/result0_1_none_0_1_rew.png} \hfill
\includegraphics[width=0.24\linewidth]{Figures/result0_1_cluster_0p01_1_rew.png} \hfill
    \includegraphics[width=0.24\linewidth]{Figures/result0_1_reward_0_1_rew.png} \hfill
    \includegraphics[width=0.24\linewidth]{Figures/result0_1_reward_0p1_1_rew.png}
    
% \vspace{-0.3cm}
\par\caption{\textbf{Cumulative rewards in MNIST}. Fixed arms: (a) stationary, $p_r$=0.01; (b) varying clusters, $p_r$=0.01; (c) negative images, $p_r$=0.1; (d) shuffled rewards, $p_r$=0.01. Extendable arms: (e) stationary, varying $p_r$; (f) varying clusters, $p_r$=0.01; (g) shuffled rewards, varying $p_r$; (h) shuffled rewards, $p_r$=0.1.}\label{fig:scores}
\vspace{-1em}
\end{figure}

\begin{table}[tbh]
\begin{minipage}{\linewidth}
      \caption{\textbf{Accuracy:} Stationary contexts with different probabilities of reward revealing}
    %   \vspace{-0.1cm}
      \label{tab:stat} 
      \centering
      \resizebox{\linewidth}{!}{
 \begin{tabular}{ l | c | c | c | c | c | c  | c | c }
 &\multicolumn{2}{c}{MNIST (varying $p_r$)} \vline & \multicolumn{2}{c}{MNIST ($p_r$=0.5)} \vline & \multicolumn{2}{c}{MNIST ($p_r$=0.1)} \vline & \multicolumn{2}{c}{MNIST ($p_r$=0.01)}   \\
  & fixed arms & extendable  & fixed arms & extendable  & fixed arms & extendable & fixed arms & extendable  \\ \hline
LinUCB & 0.1134 & 0.094 & 0.1080 & 0.0962 & 0.0842 & 0.0762  & 0.0252   &  0.0902   \\ \hline
BerlinUCB & 0.1138 & 0.0990 &  0.1102  &   0.0990 &   0.1016 &  0.0926   & 0.0788  & 0.0896      \\
B-Kmeans & 0.2594 & 0.2130 &  0.2674 &   \textbf{0.2678} &   \textbf{0.3132} &  \textbf{0.2760} &   \textbf{0.1400}   & 0.0828      \\
B-KNN & \textbf{0.2642} & \textbf{0.2398} &  \textbf{0.2722}  &    0.2642 &   0.2954 &  0.2622  &  0.1384     &  \textbf{0.0938}             \\
B-GMM & 0.0958 & 0.0768 &  0.1060  & 0.0728 & 0.0958 & 0.0320 & 0.1034  &  0.0120 \\ 
 \end{tabular}
}
 \end{minipage}
\end{table}

\begin{table}[tbh]
\begin{minipage}{\linewidth}
      \caption{\textbf{Accuracy:} Nonstationary cases with different probabilities of reward revealing}
    %   \vspace{-0.1cm}
      \label{tab:nostat} 
      \centering
      \resizebox{\linewidth}{!}{
 \begin{tabular}{ l | p{1.5cm} | p{1.5cm} | p{1.5cm} | p{1.5cm} | p{1.5cm} |p{1.5cm} | p{1.5cm} | p{1.5cm} | p{1.5cm} | p{1.5cm} | p{1.5cm} | p{1.5cm} | p{1.5cm}}
  &\multicolumn{3}{c}{MNIST - varying clusters} \vline & \multicolumn{3}{c}{MNSIT - negative images} \vline & \multicolumn{3}{c}{MNSIT - shuffled rewards}  \\
 Fixed Arms & $p_r$=0.5 & $p_r$=0.1 & $p_r$=0.01 & $p_r$=0.5 & $p_r$=0.1 & $p_r$=0.01 & $p_r$=0.5 & $p_r$=0.1 & $p_r$=0.01 \\ \hline
LinUCB &   \textbf{0.1086}   & 0.0984  &  0.0690   & 0.1044   & 0.0920  & 0.0732  & 0.1172   & 0.0832  & 0.0512  
  \\ \hline
BerlinUCB &   0.1024   &   0.1002   &   0.0828    &   0.1016  &   0.0970  &  0.1016  &   0.1120    & 0.0966 & 0.0832      \\
B-Kmeans &    0.0952    &  \textbf{0.1096}    &  \textbf{0.1074}   &   0.1082     &    0.1036  &  0.0768 & \textbf{0.2776}  &    0.2878   &  \textbf{0.1618}     \\
B-KNN &    0.0984    &   0.1002      & 0.1050 &     \textbf{0.1762}    &    \textbf{0.1732}    & 0.1016 &    0.2600      &   \textbf{0.3162}   & 0.1556   \\
B-GMM &   0.1072  &   0.0974   &  0.1034 &   0.0954 &  0.1074  &  \textbf{0.1018} & 0.1158  &   0.1172 &  0.1062      \\ 
 \end{tabular}
}
 \end{minipage} 
 \begin{minipage}{\linewidth}
    %   \caption{\textbf{Accuracy:} Nonstationary cases with different probabilities of reward revealing}
    % %   \vspace{-0.1cm}
    %   \label{tab:nostat} 
      \centering
      \resizebox{\linewidth}{!}{
 \begin{tabular}{ l | p{1.5cm} | p{1.5cm} | p{1.5cm} | p{1.5cm} | p{1.5cm} |p{1.5cm} | p{1.5cm} | p{1.5cm} | p{1.5cm} | p{1.5cm} | p{1.5cm} | p{1.5cm} | p{1.5cm}}
  &\multicolumn{3}{c}{MNIST - varying clusters} \vline & \multicolumn{3}{c}{MNSIT - negative images} \vline & \multicolumn{3}{c}{MNSIT - shuffled rewards}  \\
Extendable Arms  & $p_r$=0.5 & $p_r$=0.1 & $p_r$=0.01 & $p_r$=0.5 & $p_r$=0.1 & $p_r$=0.01 & $p_r$=0.5 & $p_r$=0.1 & $p_r$=0.01 \\ \hline
LinUCB &  0.0994   &  0.0930   &  0.0866  &  0.0888   & 0.0918   & \textbf{0.1014} & 0.1010   & 0.0872  &  0.1014  \\ \hline
BerlinUCB &    0.0930     &   0.0946    &    \textbf{0.0938}   &   0.0924    &    0.0930 &    0.0910    & 0.0994   &  0.0926 &   0.0918     \\
B-Kmeans & \textbf{0.1010}     &   \textbf{0.0990}     &     0.0380   &   0.0910    &  0.0712   &   0.0308   &     0.2478   &  0.2336   &  0.0654       \\
B-KNN &   0.0958   &  0.0970      &   0.0570  & \textbf{0.1780}     &   \textbf{0.1228}   &  0.0460    &     \textbf{0.2606}    & \textbf{0.2818}  &  \textbf{0.1016}       \\
B-GMM &    0.0756    &  0.0296  &   0.0108  &  0.0680 & 0.0338  &   0.0118 &  0.0720  &    0.0258 &   0.0180  \\ 
 \end{tabular}
}
 \end{minipage} 
 \vspace{-1em}
\end{table}


\begin{table}[tbh]
 \vspace{-1em}
\begin{minipage}{\linewidth}
      \caption{\textbf{Accuracy:} Nonstationary contexts with varying episodic rewards}
    %   \vspace{-0.1cm}
      \label{tab:nscont} 
      \centering
      \resizebox{\linewidth}{!}{
 \begin{tabular}{ l | c | c | c | c | c | c | c | c | c}
 &\multicolumn{4}{c}{varying cluster distribution} \vline & \multicolumn{4}{c}{negative images} \vline & average  \\
  & MNIST-F & MNIST-E & Warfarin-F & Warfarin-E & MNIST-F & MNIST-E & Warfarin-F & Warfarin-E \\ \hline
LinUCB & \textbf{0.1016} & 0.0946 & 0.4580 & \textbf{0.4646} & 0.0956 &  0.0912 & \textbf{0.4440} &  \textbf{0.4374}  & 0.2734  \\ \hline
BerlinUCB &  0.0986  & \textbf{0.0948} & 0.4814 &  0.4480 &   0.0988  & 0.0926 &   0.3980 &  0.3898  & 0.2628  \\
B-Kmeans & 0.1012  &  0.0944 & 0.3964 &   0.2898 &   0.1048 & 0.0854 & 0.3200 &   0.1758  & 0.1960   \\
B-KNN & 0.1012 &  0.0946 &  0.4638 &   0.4134 &   \textbf{0.1626} &  \textbf{0.1576} & 0.4188 &   0.3998   & \textbf{0.2765}  \\
B-GMM & 0.1010 &  0.0684 &  \textbf{0.5494} & 0.2208 & 0.0926 & 0.0694 &  0.3992 & 0.2002 & 0.2126  \\ 
 \end{tabular}
}
 \end{minipage}
 
\end{table}

\begin{table}[tbh]
\begin{minipage}{\linewidth}
      \caption{\textbf{Accuracy:} Nonstationary rewards with varying episodic rewards}
    %   \vspace{-0.1cm}
      \label{tab:nsrewd} 
      \centering
      \resizebox{\linewidth}{!}{
 \begin{tabular}{ l | c | c | c | c | c | c | c }
 &\multicolumn{4}{c}{shuffled class labels} \vline & \multicolumn{2}{c}{multi-task setting} \vline & average \\
  & MNIST-F & MNIST-E & Warfarin-F & Warfarin-E & MNIST/Warfarin-F & MNIST/Warfarin-E &  \\ \hline
LinUCB &   0.1080 & 0.0974 & \textbf{0.6464} & \textbf{0.6348} & 0.3496 & 0.3442 & 0.3634   
    \\ \hline
BerlinUCB &   0.1126 &    0.1036 &    0.6116 &  0.6080 & 0.3136 &  0.3071 & 0.3428
 \\
B-Kmeans &  0.2376  &    0.2566  &   0.5262  &   0.5152 &  0.3801 & 0.3690  & 0.3808    \\
B-KNN &    \textbf{0.2574} &  \textbf{0.2582} &  0.6278 &   0.6026  & \textbf{0.3833}  &   \textbf{0.4041}  & \textbf{0.4222}          \\
B-GMM &    0.0958  &  0.0664  & 0.5488 &   0.4038 &   0.2052 & 0.2375 & 0.2596 \\ 
 \end{tabular}
}
 \end{minipage}
  \vspace{-1em}
\end{table}


We explored different combinations of the above nonstationarities. Table \ref{tab:stat} summarizes our results for the setting where the contexts are stationary, we observe that BerlinUCB algorithms consistently outperforming the baseline with a large marginal ($> 20\%$ accuracy comparing to LinUCB's around $10\%$), ranked top in all 8 scenarios with different reward revealing probablity $p_r$. 

Table \ref{tab:nostat} summarizes our results for the nonstationary context due to \textit{varying cluster distribution}, data corruption with \textit{negative images}, and \textit{shuffled reward function}. As we can see, across different reward revealing probabilities $p_r$, BerlinUCB algorithms outperform the baseline on 16 out of the 18 testing scenarios. 

If we take a closer look at the nonstationary context scenarios in Table \ref{tab:nscont} where the rewards are episodically revealed with varying $p_r$ across batches, we noticed that the baseline is performing fairly well in three scenarios in Warfarin dataset. However, if we consider the mean accuracy in the entire set of this experiment, the BerlinUCB algorithms has the highest average accuracy, suggesting the advantage of using unlabelled data or missing rewards. Moreover, if we take a look at the whole iteration history, for example, for MNIST dataset (Figure \ref{fig:scores} (a)), we observe that initially, the baseline CB (orange line) is considerably worse than semi-supervised approaches, and requires a larger number of iteration to finally catch up with them. Other examples in Figure \ref{fig:scores} also demonstrated different scenarios where certain self-supervision modules (KNN and Kmeans) are more helpful than the other ones (GMM), but in most cases BerlinUCB, even without clustering modules, outperforms standard LinUCB. 

Next, Table \ref{tab:nsrewd} summarizes our results in nonstationary reward settings with \textit{shuffled reward} function and mixed domain (\textit{multi-task}) setting.
Based on the mean accuracy in the entire experiment, the top two algorithms were: B-KNN (mean accuracy  42.22$\%$) and B-Kmeans (mean accuracy 38.08$\%$). Note that, with nonstationary (shuffled) labels, the reward accumulated by the baseline CB usually remains significantly below the reward of the best semi-supervised approaches, at all iterations (Figure \ref{fig:scores}). Thus, in a more challenging setting with both context and reward nonstationarities, the semi-supervised approaches can effectively improve upon the standard contextual bandit.

We also observed an interesting phenomenon where decreasing feedback actually increases the performance in some cases (as in Table \ref{tab:nostat}). This phenomenon leads to open questions such as: What are the consequences if some feedbacks are not reliable? Can a threshold be given for the acceptable number of inaccurate feedbacks to achieve the same satisfactory level of performance? Does this behavior also exist in scenarios with non-binary reward structures? Ongoing directions include extending BerlinUCB's scalability across a series of these situations in order to better understand the full potential of the algorithm.

%  \vspace{-0.5em}
\section{Application: Interactive Speaker Recognition}
%  \vspace{-0.5em}

One important application of our online learning problem is the cold-start speaker recognition task, where new users can join a conversation at any time, and the interactive system should learn to recognize the voice profile of the newly joined user given a limited number of user feedbacks. Let's consider such an interactive speaker recognition system: At the start, there are only two buttons available:  ``No Speaker'' and ``New Speaker''. The agent chooses an arm by setting it to be highlighted. If it is correct, the user does not have to change it (unless it's ``New Speaker'', where the user needs to click on it to confirm creating a new arm). If it is incorrect, the user clicks on the right arm to give the system a feedback. 

\textbf{Application background.} Unlike synthetic online learning dataset, where a bandit feedback is always given, here in the real-life interactive systems, the user might not give the feedback timely and constantly. Note that we assume that when the agent correctly identifies the speaker (or no speaker), the user (as the feedback dispenser) should send no feedbacks to the system by doing nothing. This brings an additional layer of complexity to this application, as the agent needs to learn from a negative feedback (no feedback), assuming that it is sometimes due to a lack of timely feedback (reward not revealed) and other times due to the user's approval (reward postively revealed). In another word, in an ideal scenario when the agent does a perfect job by correctly identifying the speaker all the time, we are not necessary to be around to correct it anymore (i.e. truly feedback free). As we pointed out earlier, this could be a challenge earlier on, because other than implicitly approving the agent's choice, receiving no feedbacks could also mean the feedbacks are not revealed properly (e.g. the human oracle took a break).
To adapt BerlinUCB to this specific application, we first define our actions. There are three major classes of actions: an arm ``New'' to denote that a new speaker is detected, an arm ``No Speaker'' to denote that no one is speaking, and $N$ different arms ``User n'' to denote user $n$ speaking.
% Furthermore, we note that when ``No Speaker'' and ``User n'' arms are correctly identified, there is no feedback from us the human oracle (meaning that these arms would never have learned from a single positive reward if we don't use the ``None'' feedback iterations at all!). The semi-supervision by self-supervision step is exactly tailored for a scenario like this, where the lack of revealed positive reward for ``No Speaker'' and ``User n'' arms is compensated by the additional training of the reward mapping $\textbf{b}_{a_t}$ if context $\textbf{x}_t$ is assigned to the right arm.




% \textbf{Why is this online learning problem different?} The state-of-the-art speaker diarization systems usually require large datasets to train their audio extraction embeddings and clustering modules, especially the ones with deep neural networks and Bayesian nonparametric models. In many real-world applications in developing countries, however, the training set can be limited and hard to collect. Since these modules are pretrained, applying them to out-of-distribution environments can be problematic. For instance, an intelligent system trained with American elder speaker data might find it hard to generalize to a Japanese children diarization task because both the acoustic and contrastive features are different. To tackle this problem, we want the system to learn continually. To push this problem to the extreme, we are interested in a fully online learning setting, where not only the examples are available one by one, the agent receives no pretraining from any training set before deployment, and learns to detect speaker identity on the fly through reward feedbacks. To the best of our knowledge, this work is the first to consider diarization as a fully online learning problem. Through this work, we aim to understand the extent to which diarization can be solved as merely an online learning problem and whether traditional online learning algorithms \hfill (e.g. contextual bandits\\\cite{langford2007epoch,lin2020unified,lin2020ipd}) can be beneficial to provide a practical solution.

% \textbf{What is a preferable online speaker diarization system?} A preferable AI engine for such a realistic speaker recognition and diarization system should (1) not require user registrations, (2) allow new user to be registered into the system real-time, (3) transfer voiceprint information from old users to new ones, (4) be up running without pretraining on large amount of data in advance. While attractive, assumption (4) introduced an additional caveat that the labeling of the user profiles happens purely on the fly, trading off models pretrained on big data with the user directly interacting with the system by correcting the agent as labels. To tackle these challenges, we formulated this problem into an interactive learning model with cold-start arms and episodically revealed rewards (users can either reveal no feedback, approving by not intervening, or correcting the agent). 


\textbf{Synthetic benchmark.} We evaluated the validity of our algorithm in a synthetic online learning speaker recognition task. MiniVox \cite{lin2020speaker} is an automatic framework to transform any speaker-labelled dataset into continuous speech datastream with episodically revealed label feedbacks. This benchmark is a light-weighted environment specifically designed to simulate two real-world challenges in interactive systems: (1) the speech data in real life is never truncated into pieces for an intelligent system to classify, and (2) the reward feedbacks (i.e. telling an intelligent system that it is incorrect) is never as timely and complete. MiniVox utilizes the speaker recognition dataset like VoxCeleb \cite{Nagrani19} to create randomly generated multi-speaker ``conversations'' in continuous streams. As a proof of concept, we randomly selected 10 speaker profiles and generated a ``multi-speaker conversation'' recordings of 60000 time frames. As the industrial standard, for each time frame, we extracted the Mel Frequency Cepstral Coefficients (MFCC) \cite{hasan2004speaker} in a sliding window fashion given the real-time audio input, and it will be served as the context for our contextual bandit agents. Here we assume the number of speakers are known, and  the reward streams are sparsified given a revealing probability of 0.1, 0.01 and 0.001 to simulate different levels of users' attendance in this interactive system.
As the common metric in online learning literature, we recorded the cumulative reward: at each frame, if the agent correctly predicts a given speaker, the reward is counted as +1 (regardless of whether the agent observes the reward or not). As shown in Figure \ref{fig:results}, BerlinUCB and its variants with clustering modules consistently outperforms LinUCB in this task.


% In the working example we evaluated in this paper, we applied MiniVox on the test dataset of VoxCeleb \cite{Nagrani19} to create randomly generated multi-speaker ``conversations'' in continuous streams.
% Unlike other dataset and evaluation pipelines in speaker recognition (e.g. VoxCeleb \cite{Nagrani17}, SITW \cite{mclaren2016speakers}) and speaker diarization (e.g. CALLHOME American English \cite{canavan1997callhome}, NIST RT-03 English CTS \cite{martin2000nist}), \textit{MiniVox} environment can generate infinite length of sequences of multi-speaker conversations, and reveal rewards in an episodic fashion. 
% \subsection{Online Learning Training Pipeline}


\begin{figure}[tb]
\centering
% \vspace{-0.2cm}
    \includegraphics[width=0.3\linewidth]{Figures/vox1_mfcc_c10_0p1_rew.png} \hfill
    \includegraphics[width=0.3\linewidth]{Figures/vox1_mfcc_c10_0p01_rew.png} \hfill
    \includegraphics[width=0.3\linewidth]{Figures/vox1_mfcc_c10_0p001_rew.png}
\vspace{-0.3cm}
\par\caption{\textbf{Cumulative rewards in MiniVox}. (a) $p_r$=0.1; (b) $p_r$=0.01; (c) $p_r$=0.001.}\label{fig:results}
\vspace{-1em}
\end{figure}


This application (as demostrated in \cite{lin2020voiceid}) provides an intriguing example of how our online learning algorithm can enable an interactive system to learn to recognize speaker identity (1) entirely escaping the necessity of registering user voiceprint beforehands, (2) effortlessly incorporating new users under an optimal exploration-exploitation trade-off, (3) effectively transferring representation of registered user features to new users, and (4) continually learning despite minimal involvement of human corrections (i.e. sparse and episodic feedbacks). 
